Being Corrupt Requires Being Clever, But Detecting Corruption Doesn't

We consider a variation of the problem of corruption detection on networks posed by Alon, Mossel, and Pemantle '15. In this model, each vertex of a graph can be either truthful or corrupt. Each vertex reports about the types (truthful or corrupt) of all its neighbors to a central agency, where truthful nodes report the true types they see and corrupt nodes report adversarially. The central agency aggregates these reports and attempts to find a single truthful node. Inspired by real auditing networks, we pose our problem for arbitrary graphs and consider corruption through a computational lens. We identify a key combinatorial parameter of the graph $m(G)$, which is the minimal number of corrupted agents needed to prevent the central agency from identifying a single truthful node. We give an efficient (in fact, linear time) algorithm for the central agency to identify a truthful node that is successful whenever the number of corrupt nodes is less than $m(G)/2$. On the other hand, we prove that for any constant $\alpha > 1$, it is NP-hard to find a subset of nodes $S$ in $G$ such that corrupting $S$ prevents the central agency from finding one truthful node and $|S| \leq \alpha m(G)$, assuming the Small Set Expansion Hypothesis (Raghavendra and Steurer, STOC '10). We conclude that being corrupt requires being clever, while detecting corruption does not. Our main technical insight is a relation between the minimum number of corrupt nodes required to hide all truthful nodes and a certain notion of vertex separability for the underlying graph. Additionally, this insight lets us design an efficient algorithm for a corrupt party to decide which graphs require the fewest corrupted nodes, up to a multiplicative factor of $O(\log n)$.

==> conclusion.tex <==
\section{Conclusion}
We conclude that the condition to find a good vertex in PMC model is relaxed from the graph expander condition needed for finding most nodes. However, deciding how many bad nodes can a graph tolerate is NP-hard, and SSE-hard to approximate within any constant factor. The problem is approximated by a quantity related to $k$-vertex separator within a constant of $2$. However, since bad agents may need to go through finding k-vertex separator to find an close to optimal strategy for corrupt the graph, the task of preventing the identification of the good nodes is NP-hard for the bad nodes even approximately.

However, on the reverse side, if one is asked to devise an algorithm to find the good node if it is feasible to find, simple algorithm of finding connected component of size larger than the remaining bad nodes after removing nodes that are for sure bad would be sufficient and efficient.
\gnote{We should brainstorm open problems here.}
\begin{itemize}
\item Stronger version of hardness result not assuming SSE?
\item 
\end{itemize}


